Words are Malleable: Computing Semantic Shifts in Political and Media Discourse

Recently, researchers started to pay attention to the detection of temporal shifts in the meaning of words. However, most (if not all) of these approaches restricted their efforts to uncovering change over time, thus neglecting other valuable dimensions such as social or political variability. We propose an approach for detecting semantic shifts between different viewpoints--broadly defined as a set of texts that share a specific metadata feature, which can be a time-period, but also a social entity such as a political party. For each viewpoint, we learn a semantic space in which each word is represented as a low dimensional neural embedded vector. The challenge is to compare the meaning of a word in one space to its meaning in another space and measure the size of the semantic shifts. We compare the effectiveness of a measure based on optimal transformations between the two spaces with a measure based on the similarity of the neighbors of the word in the respective spaces. Our experiments demonstrate that the combination of these two performs best. We show that the semantic shifts not only occur over time, but also along different viewpoints in a short period of time. For evaluation, we demonstrate how this approach captures meaningful semantic shifts and can help improve other tasks such as the contrastive viewpoint summarization and ideology detection (measured as classification accuracy) in political texts. We also show that the two laws of semantic change which were empirically shown to hold for temporal shifts also hold for shifts across viewpoints. These laws state that frequent words are less likely to shift meaning while words with many senses are more likely to do so.

==> LinearMapping.tex <==
% !TEX root = ./main.tex

\section*{Linear Mapping: Methods and Results}

This idea is based on the method proposed in \cite{mikolov-mapping-2013} for learning a mapping between embeddings. In this approach we use a set of words with their extracted vectors in two embedding spaces to learn a mapping between two embedding spaces. So we have a set of training words and their vectors in two embedding spaces: $\{w_i, v_{w_i}^{E_1}, v_{w_i}^{E_2}\}_{i=1}^n$. Where $w_i$ is a word, $v_{w_i}^{E_1}$ is the vector of wiin the first embedding space and $v_{w_i}^{E_2}$ is its vector in the second embedding space. The goal is given these training samples learn a mapping from the first embedding space to the second embedding space (or the other way around). Then we can use this mapping to first map a word from one embedding to the other and then calculate the similarity of the mapped vector with the original vector for the word in the mapped embedding. If the similarity value is high, then the word has high value of stability. To learn the mapping we use gradient descent algorithm. The objective function is:
\begin{equation}
\underset{a}{\mathrm{argmin}} \sum_{i=1}^{n} (a * v_{w_i}^{E_1} - v_{w_i}^{E_2})^2
\end{equation}
where $a$ is the mapping we want to train. We define $f(x) = a * x$ ($f: E_1 \rightarrow E_2$). We learn the mapping using gradient descent algorithm. Finally, we define two measures of stability of words using the linear mapping method:
\begin{itemize}
\item One-way stability measure: We define the one-way stability measure of a word $w$ as:
\begin{equation}
S(w) = cosine(f(v_{w}^{E_1}), v_{w}^{E_2})
\end{equation}
\item Two-way stability measure: We define the two-way stability measure of a word $w$ as:
\begin{equation}
S(w) = cosine(g(f(v_{w}^{E_1})), v_{w}^{E_1})
\end{equation}
where $f$ is defined abow. Similar to $f$, $g$ is also a mapping learned using gradient descent, but $g: E_2 \rightarrow E_1$. 
\end{itemize}

\begin{table}[h]
    \centering 
    \caption{\label{table:1} The results of linear mapping methods} 
    \begin{tabular}{c c c}
    \toprule
    Setting & One-way & Two-way \\
    \hline
    $E_1= Con, E_2=Lab$ & 0.427 & 0.843 \\
    $E_1= Lab, E_2=Con$ & 0.434 & 0.848\\
    \bottomrule
    \end{tabular}
\end{table}



==> NeighbourBasedMethod.tex <==
% !TEX root = ./main.tex

\section{Neighbour Based Word Stability: Methods and Results}

The main assumption of this method is that a word is stable if it has similar neighbouring words in both embeddings. Thus, the stability of a word can be calculated based on the similarity of its neighbours in two embeddings. Based on this assumption, we define a familiy of stability metric as:
\begin{equation}
\label{NeighBasedMetric}
S(w) = sim(w, N_w^{E1}, N_w^{E2}), 
\end{equation}
where $N_w^{Ei}$ is the neighbours of $w$ in embedding $Ei$. $N_w^{Ei}$ is achieved by taking top $m$ most similar words to $w$ in embedding space $Ei$. We define different neighbour based metrics using Equ. \ref{NeighBasedMetric}. 

\subsection{Measure1}
The first measure is an iterative method. The main assumption is that a word is more stable if it has similar neighours in both embeddings and those neighbours themself are stable. This measure is defined as:
\begin{equation}
S^t(w) = \frac{sim^t(v_w^{E1}, N_w^{E2}) + sim^t(v_w^{E2}, N_w^{E1})}{2},
\end{equation}
where $v_w^{Ei}$ is the vector of $w$ in embedding $Ei$ and $S^t(w)$ is the stability of $w$ at iteration $t$. $sim^t(v_w^{E1}, N_w^{E2})$ is defined as follows:
\begin{equation}
sim^t(v_w^{E1}, N_w^{E2}) = \frac{1}{|N_w^{E2}|} \sum_{w' \in N_w^{E2}} cosine(v_w^{E1}, v_{w'}^{E1}) * S^{t-1}(w'),
\end{equation}

We first suppose that all words are stable and set $S(w)=1$ for all words. At first iteration, only direct neighbours contribute to the stability of words. At iteration $t=k$, the undirect neighbours accessible by $k$ edges in the graph contribute to the stability of words. After each iteration we re-scale the stability values to fall into [0, 1] interval.
